Parameter Synthesis Problems for one parametric clock Timed Automata

In this paper, we study the parameter synthesis problem for a class of parametric timed automata. The problem asks to construct the set of valuations of the parameters in the parametric timed automa- ton, referred to as the feasible region, under which the resulting timed automaton satisfies certain properties. We show that the parameter syn- thesis problem of parametric timed automata with only one parametric clock (unlimited concretely constrained clock) and arbitrarily many pa- rameters is solvable when all the expressions are linear expressions. And it is moreover the synthesis problem is solvable when the form of con- straints are parameter polynomial inequality not just simple constraint and parameter domain is nonnegative real number.

==> SVM.tex <==
% !Mode\dots ``TeX:UTF-8''
\subsection{Decidable results}
In general, when there is only one clock which has guard or invariants with parameter then 
the {\em Problem \ref{pro:synth}} is decidable; if there are more than two clocks which has 
guard or invariant with parameter then the {\em Problem \ref{pro:synth}} is undecidable~ \cite{alur1993parametric}. In \cite{HUNE2002183}, the authors provide a subclass of \pta\
which called {\em lower bound/upper bound (L/U) automata}, they prove that the {\em emptiness problem} is decidable for this kind a automata.  In the follows, we will extends~\cite{HUNE2002183} result, and prove that if there are no guards and invariants with parameters has form $f=e$, then the {\em emptiness problem} is decidable.

\subsection{Lower bound/upper bound automata}
Informally, each parameter in an L/U automata $\TA$ occurs either as a lover bound in the invariants and guards of $\TA$ or as an upper bound, but never as both. For instance, $p$ is a \upp\ in $x-y< 2p$ and  $x-y< 2p$ is a \pup. Lower bound parameters are for instance $p_1$ and $p_2$ in $y-x> p_1+3p_2$ and  $x-y< 2p-p_1-2p_2$, $y-x> q_1+3p_2$ is  called \plb . A PTA containing both the guards $x-y\le p-p_1$ and $z< p_1-p$ is not an L/U automata.

\begin{definition}[L/U]\cite{HUNE2002183}
	A parameter $p_i\in P$ is said to occur in the linear expression $e=a_0+a_1p_1+\cdots+a_np_n$ if $a_i\neq 0$; $p_i$ occurs positively in $e$ if $a_i>0$ and $p_i$ occurs negatively in $e$ if $a_i<0$. 
	A lower bound parameter of PTA $\TA$ is a paramter that only occurs negatively in the expressions of $\TA$ and an upper bound parameter of $\TA$ is  a parameter that only occurs positively in $\TA$. We call $\TA$ a lower bound/upper bound (L/U) automata if  every parameter occurring in $\TA$ is either a lower bound parameter or an upper bound parameter.
	
\end{definition}

Hence, in the L/U automata the parameters are divided  into two class $L$ and $U$ which are lover bound parameters and upper bound parameters,  respectively. For a parameter valuation $\gamma$ 
we also divide it into parts $\gamma_l,\gamma_u$ which corresponding $L$ and $U$.  Furthermore, we consider, apart from parameter valuation is a parameter valuation with values in 
$\NN\cup \{\infty\}$, rather than in $\RR$. Extended parameter valuations are useful in certain  cases to solve the verification problem. Working with extended parameter valuations may cause the 
evaluation of expression to be undefined. For example, the expression $e[\gamma]$ is not defined for $e=q_1-q_2$ and $\gamma[p_1]=\gamma[p_2]=\infty$. We therefore require that an extended parameter  valuation does not assign the $\infty$ to both a lower bound parameter and an upper bound  parameter. Here, we use the conventions that $0\infty=0$, than $x- y\prec \infty$ evaluates to
true and $x-y\prec -\infty$ to false. The parameter valuation $[0,\infty]$ denote that assign $0$ for each lower bound parameter and assign $\infty$ to each upper bound parameter. 


\begin{proposition}[\cite{HUNE2002183}]
	\label{prop:eq}
	Let $\TA$ be a L/U automata and $\phi$ a state formula. Then
	\begin{enumerate}
		\item  $[[\TA[\gamma_l,\gamma_u]]]\models \exists \Diamond \phi \Longleftrightarrow \forall \gamma_l'< \gamma_l, \gamma_u< \gamma_u':[[\TA[\gamma_l',\gamma_u']]]\models\exists \Diamond \phi. $
		\item $[[\TA[\gamma_l,\gamma_u]]]\models \forall \Box \phi \Longleftrightarrow \forall \gamma_l< \gamma_l', \gamma_u'< \gamma_u:[[\TA[\gamma_l',\gamma_u']]]\models\forall \Box \phi. $
	\end{enumerate}
\end{proposition}
	
\begin{corollary}[\cite{HUNE2002183}]
		The {\em emptiness problem} is decidable for L/U automata.
\end{corollary}

==> twoPTA.tex <==
% !Mode\dots ``TeX:UTF-8''
\section{Two parametrically constrained clocks and one parameter case}
\label{sec:twoC}

%\begin{theorem}[Computable]
%	Let $\TA$ be an L/U \pta\ with one parameter $p$. If $\psi$ be  $\exists \Diamond \phi$, then set $\Gamma(\TA,\psi)$ is solvable.
%\end{theorem}
%
%\begin{proof}
%	Proofs by induction.
%	Let $H$ be $\Gamma(\TA, \psi)$.
%	Let $n$ be the number of parametrically constrained clock. When $n=1$, by {\em Proposition \ref{prop:new10}}, the   conclusion holds.
%	
%	Assume that the conclusion holds when $n\le K$.  When $n=K+1$. 
%	
%	
%	If $p_{K+1}$ is a lower bound parameter, let $p_{K+1}=0$ in $\TA$, obtain a 
%	new PTA $\TA'$. By the assumption, we can compute the entire set of 
%	parameter valuation which make  $[[\TA'[\gamma]]]\models \exists \Diamond \phi$ satisfy. If the solution set of $\TA'$ is empty, then through {\em Proposition \ref{prop:eq}}, $H=\emptyset$.  Otherwise, 
%	let $T$ be max upper bound of  concretely constrained clocks. Let $p_{M+1}=T+1$ in $\TA$, obtain a new PTA $\TA''$. By the assumption, we can compute the entire set of 
%	parameter valuation which make  $[[\TA''[\gamma]]]\models \exists \Diamond \phi$ satisfy. 
%	\qed
%\end{proof}
%\begin{corollary}\label{cor:new10}
%		Let $\TA$ be a \pta\  with one parameter $p$. 
%		Let $\psi$ be  $\forall \Box \phi$. Then set $\Gamma(\TA,\psi)$ is computable.
%\end{corollary}

%
%\begin{theorem}[L/U computable]
%	Let $\TA$ be an L/U automata. Let $\psi$ be  $\exists \Diamond \phi$. Then set $\Gamma(\TA,\psi)$ is computable.
%\end{theorem}
%\begin{corollary}\label{cor:new1}
%		Let $\TA$ be an L/U automata. Let $\psi$ be  $\forall \Box \phi$. Then set $\Gamma(\TA,\psi)$ is computable.
%
%\end{corollary}


For a PTA $\TA$, we use $C^s_{\TA}$  is the sum of  $\{|c|\mid \mbox{ there is a concretely  expression} \\  \mbox{ of }  \TA \mbox{ of the form } c_0\mbox{ and } c=c_0 \}$.  
 Let $C_s=2C_{\TA}^0+C^s_{\TA}+C_{\psi}+1$.

\begin{lemma}
	\label{lem:newp2}
	Let $\TA$ be a \pta\ with two parametrically constrained clocks  $x,y$ and one parameter $p$. Let $\psi$ be $\exists \Diamond \phi$.  If there is a $T_1\ge C_s$ such that  $[[\TA[\{p=T_1\}]]]\models  \psi$, then  $[[\TA[\{p=T\}]]]\models  \psi$ for $T\ge C_s$.
\end{lemma}

\begin{proof}
		Let parameter valuation $\gamma=\{p=T_1\}$.
		By {\em Lemma \ref{lem:moveP}}, without loss of generation we set $\phi$ be $q_N$.
		Let $\tau$ be $s_0a_1s_1\cdots a_Ns_N$ and $s_i=(q_i,\omega_i)$ be a run such that satisfies property $\psi$.  Let $\tau_1=q_0a_1q_1\cdots a_Nq_N$.  We can obtain a run $\tau'$ by the method of {\em Lemma \ref{lem:moveI}} where $\tau'$ satisfies that  $R(\tau')\neq \emptyset \Longleftrightarrow R(\tau_1)\neq \emptyset $  for each parameter valuation $\gamma$ and $\tau'$ without location invariant. 
		
		% In run $\tau'$ we obtain $\tau''$ through update the parameter valuation by $T_2$.  By {\em Lemma \ref{lem:up}}, $R(\tau'')\neq \emptyset$
		% for each parameter valuation $p\in \{0,1,\cdots\}$.
		
		Let $k$ be the number of \plb\ on $\tau'$.   We proof by induction $k$.
		If $k=0$, we obtain $\tau_1$ through  updating \tl{  $\omega_i(x)=\max\{C_{\TA}^0,C_{\psi}\}+1$ if $\omega_i(x)> \max\{C_{\TA}^0,C_{\psi}\}+1$.} Then it is 
		easy to check that $\tau_1$ satisfies $\psi$ under parameter valuation $p=C$.  By {\em Proposition \ref{prop:monot}}, $R(\tau')\neq \emptyset$  for each parameter valuation $\gamma=\{p=T\}$ where $T\ge C_s$. In other words,  the conclusion holds.
		
		When $k=1$. Let $a_i'$
		be the  discrete transition of $\tau'$ whose guard has  one  conjunctive component  with \plb. 
		
		If this  conjunctive component  is form $x\succ e$ where the coefficient of $p$ in $e$ is positive.  When there is a conjunctive component
		of $a_i'$ guard with form $x\prec e_1$ where  the coefficient of $p$ in $e_1$ is positive. Since there is  $x$ such that $\left(x\succ e\right)\wedge \left(x\prec e_1 \right)$ is feasible  when $p=T_1$. Thus, $p=T_1\models (e_1-e\ge 0)$. Let $c_1,c_2$ be the constant occurring in $e,e_1$, respectively. By the definition of $C_{s}$, $C_{s}> |c_1|+|c_2|+1$, hence $T_1> |c_1|+|c_2|+1 $. Thus, the coefficient of $p$ in expression $e_1-e$ is a nonnegative integer. Therefore,   $p=T\models (e_1-e\ge 0)$ for $T\ge C_{s}$.
		Furthermore, if  $p=T_1\models (e_1-e> 0)$, then  $p=T\models (e_1-e> 0)$ for $T\ge C_{s}$ and $p=T_1\models (e_1-e= 0)$, then  $p=T\models (e_1-e= 0)$ for $T\ge C_{s}$. 
		 What is means, formula  $ \left(x\succ e\right)\wedge \left(x\prec e_1 \right)$ is feasible when $T\ge C_s$.
		
		Assume the conclusion holds when $k\le K$ where $K\ge 1$.
		
		When $k=K+1$. Let $a_i'$
		be the last discrete transition of $\tau'$ whose guard has  one  conjunctive component  with \plb, and  $a_j'$
		be the  transition of $\tau'$ which right next to $a_i'$ and its  guard has  one  conjunctive component  with \plb . 
		
		If this  conjunctive component  is form $x\succ e$ where the coefficient of $p$ in $e$ is positive.  When there is a conjunctive component
		of $a_i'$ guard with form $x<(\le)e_1$ where  the coefficient of $p$ in $e_1$ is positive. Since there is  $x$ such that $\left(x>(\ge)e\right)\wedge \left(x<(\le)e_1 \right)$ is feasible  when $p=T_1$. Thus, $p=T_1\models (e_1-e>1)$. let $c_1,c_2$ be the constant occurring in $e,e_1$, respectively. By the definition of $C_{s}$, $C_{s}> |c_1|+|c_2|+1$. Thus, the coefficient of $p$ in expression $e_1-e$ is positive. Therefore,   $p=T\models (e_1-e>1)$ for $T\ge C_{s}$. What is means, formula  $ \left(x>(\ge)e\right)\wedge \left(x<(\le)e_1 \right)$ is feasible when $T\ge C$.
		
	\qed
\end{proof}


\begin{theorem}[Two parameter clocks]
	Let $\TA$ be a \pta\ with two parameter clocks $x,y$ and one parameter $p$. Let $\phi$ be a  property. If  $\psi$ be $\exists \Diamond \phi$, then set $\Gamma(\TA,\psi)$ is solvable.
\end{theorem}


==> twoone.tex <==
% !Mode\dots ``TeX:UTF-8''
% !TEX root = ../paratmp.tex

\section{Parametric timed automata with two parametric clocks and one paramter}
\label{sec:two}
 In this section, we present our other contribution and the solution to the   {\em parameter synthesis problem} of PTAs  with two parametric clocks $x,y$ and one parameter $p$ and the
  {\em atomic constraints} of the form which we consider 
in this section are  $b_1x-b_2y\prec p$ and $b_1x-b_2y\succ p$  where 
$\prec \in \{<,\le\},\succ \in \{>,\ge\}$ and $b_1,b_2\in \{0,1\}$, which we call   {\em two-one PTAs}. In this section, parameter values $\PP=\NN$.
All the form of atom constraints can list in {\em Table \ref{tab:1}}.
\begin{table}
\begin{center}


\begin{tabular}{|c|c|c|c|}
	\hline
	$x\prec c$ 	& $x\prec p$ 	&	$x\succ c$ 	& $x\succ p$ \\
	\hline
	$y\prec c$ 	& $y\prec p$ 	&  	$y\succ c$ 	& $y\succ p$ \\    
	\hline
	$-x\prec c$ 	& $-x\prec p$ 	&	$-x\succ c$ 	& $-x\succ p$ \\
	\hline
	$-y\prec c$ 	& $-y\prec p$ 	&  	$-y\succ c$ 	& $-y\succ p$ \\    
	\hline
	$x-y\prec c$ 	& $x-y\prec p$ 	&	$x-y\succ c$ 	& $x-y\succ p$ \\     
	\hline
	$y-x\prec c$ 	& $y-x\prec p$ 	&	$y-x\succ c$ 	& $y-x\succ p$\\
	\hline
\end{tabular}
\end{center}
\caption{All possible atom constraint forms in two-one PTA}
\label{tab:1}
\end{table}
 An  two-one PTA allows an arbitrarily number of  {\em concretely constrained clocks}, and we denote an two-one PTA $\mathcal{A}$ with the parametric locks $x,y$ and parameter $p$ as $\TA[(x,y),p]$, and as $\mathcal{A}$ when there is no confusion. We use $\mathcal{A}[p=v]$ for the LTS (and the concrete PTA) under the valuation $p=v$, and as $\TA[v]$ when there is no confusion. Our main theorem is that the entire set of feasible parameter valuations $\Gamma(\mathcal{A}[(x,y),p], \psi)$  is computable for any two-one PTA $\mathcal{A}[(x,y),p]$ and any system property $\psi$ defined. The theorem is formally stated below.


\begin{theorem}[Synthesisability of two-one PTA]
\label{th:two-one-PTA}
	 The set $\Gamma(\TA,\psi)$  of feasible parameter valuations is solvable  for any two-one PTA $\mathcal{A}[(x,y),p]$ and any system property $\psi$.
\end{theorem}
In order to prove {\em Theorem \ref{th:two-one-PTA}}, we will list some notations and list some lemmas.

For a PTA $\TA$, we use  $\maxC(\TA)$   to denote the maximum of the absolute values of the constant terms occurring in the linear expressions of $\TA$, that is, 
 \[\maxC(\TA)\deff \max\{|\textit{con}(e)| \mid  e\in \textit{expr}(\TA)\}. \]  
 We use $K$ to denote the number of transitions in $\TA$.
For a property $\psi$, we use $\textit{maxV}(\psi)$  to denote the maximum of absolute value of the constants which occur in $\psi$, and we define the constant 
\[S_0\deff 2K\cdot \max\{\textit{maxC}({\TA}),\maxV(\psi)\}+1\] and
\[S_1\deff 4S_0.\]


\begin{lemma}
	\label{lem:oneP1}
	For a  a  syntactic  run   $\tau$ of a two-one PTA $\mathcal{A}[(x,y),p]$ where $\tau$ without clocks reset,   we have $R(\mathcal{A}_\tau[p=T])\neq \emptyset$ for any $T\ge S_1$ if there is a $T_1\ge S_1$ such that $R(\mathcal{A}_\tau[p=T_1])\neq \emptyset$.
\end{lemma}

\begin{proof}
 Let $\xi= (q_0{,}\omega_0)\xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_\ell} (q_\ell{,}\omega_\ell)$ be one of run of $\tau$.
Since there is no clocks reset in $\tau$, the values of clocks $x$ and $y$ keep  changing synchronously in each run of $\tau$. Hence, there is no
conjunct of guard in  $\tau$ with form of $x-y\succ p$ or $y-x\succ p$.  In other words,  the possible form of  parametric constraints  in $\tau$ is
upper bound $x\prec p$, $y\prec p$, $x-y\prec p$ or $y-x\prec p$. We update run $\xi$ by  $\omega_i(x)=\omega_i(y)=S_1-1$ if $ \omega_i(x)> S_1$.  Since there is a no constant number in $\tau$ greater than
$\frac{S_1}{2}$, the new $\xi$ satisfies every concrete constraint in $\tau$ and the  form of parametric atomic constraints is $x\prec p$ or $y\prec p$ in $\tau$.
Thus, $\xi$ is 
a run for $\tau[p=T]$ when $T\ge S_1$. Therefore, the conclusion holds.
\qed
\end{proof}



\begin{lemma}
\label{lem:oneP3}
Let $\tau=(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_\ell\&a_\ell[u_\ell]}(q_\ell,true)
$ be a  syntactic run of  PTA $\TA[(x,y),p]$ and $\gamma$ is a parameter valuation.
If there is a run
 \[\xi= (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_\ell} (q_\ell{,}\omega_\ell)\]
  of $\tau[\gamma]$ such that 
$\omega_\ell(x)-\omega_\ell(y)\ge S_1$, then  there is a pair   $0\le i\le j < \ell$ such that 
\begin{enumerate}
\item $\omega_i(x)< S_0\wedge \omega_{i+1}(x)\ge S_0$;
\item $\omega_j(x)< 3S_0\wedge \omega_{j+1}(x)\ge 3S_0$;
\item there is a clocks reset about clock $y$ in $u_k$ where $k\in (i,\ell]$;
\item there is no clocks reset about clock $x$ in $u_k$ where $k\in (i,\ell]$;
\item there is no conjunct of $g_k$ with  parameter-free atomic constraints $ x\prec c $   where $k\in (i,\ell]$.
\end{enumerate}
 \end{lemma}
 
\begin{proof}
Since $\omega_\ell(x)-\omega_\ell(y)\ge S_1$ and $\omega_\ell(y)\ge 0$, $\omega_\ell(x)\ge S_1$. As 
$\omega_{\ell}(x)=\left(\omega_{\ell-1}'[u_{\ell}]\right)(x)$, 
every constant occurring in $\TA$ is less than $S_0$ and $\omega_{\ell}(x)\ge S_0$, there is no clock reset of $x$ in $u_{\ell}$ and there is no  parameter-free atomic constraints $ x\prec c $ in $g_\ell$.
 Thus, $
\omega_\ell(x)=\omega_{\ell-1}'(x)$.
Since $\omega_{\ell-1}'(x)\ge \omega_{\ell-1}(x)$, $\omega_\ell(x)\ge \omega_{\ell-1}(x)$. 

If $\omega_{\ell-1}(x)\ge 3S_0$, repeating above procedure
 until find the $j$ such that $\omega_{j}(x)< 3S_0$. 
 If $\omega_{j}(x)< S_0$, let $i=j$, else repeating above procedure
 until find the $i$ such that $\omega_{i}(x)< S_0$. Then  $\omega_k(x)\le \omega_{k+1} (x)$  and  $\omega_{k+1}(x)= \omega'_{k} (x)$ for $k\in [i,\ell)$.
 In other words, there is no  clocks reset about clock $x$ in $u_k$  and there is no  parameter-free atomic constraints $ x\prec c $ in $g_k$ for $k\in (i,\ell]$.
 Since $\omega_i(y)\ge 0$, $\omega_i(x)-\omega_i(y)< S_0$. 
 
 
 Assume that there is no  clocks reset about clock $y$ in $u_k$ where $k\in (i,\ell]$. Then $x$ and $y$ keep  changing synchronously during
  $a_{i+1},\cdots,a_{\ell}$. So
 $\omega_\ell(x)-\omega_\ell(y)= \omega_i(x)-\omega_i(y)< S_0$, which contracts with $\omega_\ell(x)-\omega_\ell(y)\ge 4S_0$. Hence the assumption can not hold and
 there is a  clocks reset about clock $y$ in $u_k$ where $k\in (i,\ell]$. 
\qed
\end{proof}
\begin{table}
	\begin{center}	
		\begin{tabular}{|c|c|c|c|}
			\hline
			\cellcolor[gray]{0}
			$x\prec c$ 	& $x\prec p$ 	&	$x\succ c$ 	& $x\succ p$ \\
			\hline
			$y\prec c$ 	& $y\prec p$ 	&  	$y\succ c$ 	& $y\succ p$ \\    
			\hline
			$-x\prec c$ 	& $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 	  $-x\succ p$ \\
			\hline
			$-y\prec c$ 	& $-y\prec p$ 	&  	$-y\succ c$ 	& 	$-y\succ p$ \\    
			\hline
			$x-y\prec c$ 	& $x-y\prec p$ 	&	$x-y\succ c$ 	& $x-y\succ p$ \\     
			\hline
			$y-x\prec c$ 	& $y-x\prec p$ 	&	$y-x\succ c$ 	& $y-x\succ p$\\
			\hline
		\end{tabular}
	\end{center}
	\caption{All possible atom constraint forms of guard $g_j$ for $j \in (i,\ell]$ in {\em Lemma \ref{lem:oneP3}}}
	\label{tab:2}
\end{table}



\begin{lemma}
	\label{lem:oneP5}
	Let $\tau=(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_\ell\&a_\ell[u_\ell]}(q_\ell,true)
	$ be a  syntactic run of  PTA $\TA[(x,y),p]$ and $\gamma$ is a parameter valuation.
	If there is a run
	\[\xi= (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_\ell} (q_\ell{,}\omega_\ell)\]
	of $\tau[\gamma]$ such that 
	$\omega_\ell(y)-\omega_\ell(x)\ge S_1$, then  there is a pair $0\le i\le j<  \ell$ such that 
	\begin{enumerate}
		\item $\omega_i(y)< S_0\wedge \omega_{i+1}(y)\ge S_0$;
		\item $\omega_j(y)< 3S_0\wedge \omega_{j+1}(y)\ge 3S_0$;
		\item there is a clocks reset about clock $x$ in $u_k$ where $k\in (i,\ell]$;
		\item there is no clocks reset about clock $y$ in $u_k$ where $k\in (i,\ell]$;
		\item there is no conjunct of $g_k$ with  parameter-free atomic constraints $ y\prec c $   where $k\in (i,\ell]$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	As clocks $x$ and $y$ are symmetrical in $\TA$.  Hence, employing  the proof of {\em Lemma \ref{lem:oneP3}}, we can prove this lemma.
\qed	
\end{proof}

\begin{table}
\begin{center}
	\begin{tabular}{|c|c|c|c|}
		\hline
		$x\prec c$ 	& $x\prec p$ 	&	$x\succ c$ 	& $x\succ p$ \\
		\hline
		\cellcolor[gray]{0}
		$y\prec c$ 	& $y\prec p$ 	&  	$y\succ c$ 	& $y\succ p$ \\    
		\hline
		$-x\prec c$ 	& $-x\prec p$ 	&	$-x\succ c$ 	& 	 $-x\succ p$ \\
		\hline
		$-y\prec c$ 	& $-y\prec p$ 	&  		\cellcolor[gray]{0} $-y\succ c$ 	& 		  $-y\succ p$ \\    
		\hline
		$x-y\prec c$ 	& $x-y\prec p$ 	&	$x-y\succ c$ 	& $x-y\succ p$ \\     
		\hline
		$y-x\prec c$ 	& $y-x\prec p$ 	&	$y-x\succ c$ 	& $y-x\succ p$\\
		\hline
	\end{tabular}
\end{center}
\caption{All possible atom constraint forms of guard $g_j$ for $j \in (i,\ell]$ in {\em Lemma \ref{lem:oneP5}}}
\label{tab:3}
\end{table}


\begin{lemma}
	\label{lem:oneP6}
	Let $\tau=(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_\ell\&a_\ell[u_\ell]}(q_\ell,true)
	$ be a  syntactic run of  PTA $\TA[(x,y),p]$ and $\gamma$ is a parameter valuation.
	If there is a run
	\[\xi= (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_\ell} (q_\ell{,}\omega_\ell)\]
	of $\tau[\gamma]$ such that 
	$\omega_\ell(x)\ge S_1$  and $\omega_\ell(y)\ge S_1$, then  there is a  $0\le i<  \ell$ such that 
	\begin{enumerate}
		\item $\omega_{i+1}(x)\ge 3S_0\wedge \omega_{i+1}(y)\ge 3S_0$;
		\item there is no clocks reset about clocks $x,y$ in $a_j$ where $j\in (i,\ell]$;
		\item there is no conjunct of $a_j$ with  parameter-free atomic constraints  $x\prec c$ and $ y\prec c $   where $j\in (i,\ell]$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	Since $\omega_\ell(x)\ge S_1$, $\omega_{\ell}(x)=\left(\omega_{\ell-1}'[u_{\ell}]\right)(x)$ and
	every constant occurring in $\TA$ is less than $S_0$, there is no clock reset of $x$ in $u_{\ell}$ 
	and there is no  conjunct of $g_\ell$ with 
	parameter-free atomic constraints  $x\prec c$.
	Thus, $
	\omega_\ell(x)=\omega_{\ell-1}'(x)$.
	Since $\omega_{\ell-1}'(x)\ge \omega_{\ell-1}(x)$, $\omega_\ell(x)\ge \omega_{\ell-1}(x)$. 
	
	If $\omega_{\ell-1}(x)\ge 3S_0$, repeating above procedure
	until find an $i_1$ such that $\omega_{i_1}(x)< 3S_0$. Then  $\omega_j(x)\le \omega_{j+1} (x)$  and  $\omega_{j+1}(x)= \omega'_{j} (x)$ for $j\in [i_1,\ell)$.
	In other words, there is no  clocks reset about clock $x$ in $a_j$ and there is no  conjunct of $g_j$ with 
	parameter-free atomic constraints  $x\prec c$ where $j\in (i_1,\ell]$.
	
	By the same reason we can choose an $i_2$ such that 
	\begin{enumerate}
			\item $ \omega_{i_2+1}(y)\ge 3S_0$;
			\item there is no clocks reset about clocks $y$ in $u_j$ where $j\in (i_2,\ell]$;
			\item there is no conjunct of $g_j$ with  parameter-free atomic constraints $ y\prec c $   where $j\in (i_2,\ell]$.
	\end{enumerate}
	
	Let $i=\max\{i_1,i_2\}$, then 
		\begin{enumerate}
			\item $\omega_{i+1}(x)\ge 3S_0\wedge \omega_{i+1}(y)\ge 3S_0$;
			\item there is no conjunct of $g_j$ with  parameter-free atomic constraints  $x\prec c$ and $ y\prec c $   where $j\in (i,\ell]$;
			\item there is no clocks reset about clocks $x,y$ in $u_j$ where $j\in (i,\ell]$.
		\end{enumerate}
\qed
\end{proof}


\begin{lemma}
	\label{lem:oneP7}
	Let $\tau=(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_\ell\&a_\ell[u_\ell]}(q_\ell,true)
	$ be a  syntactic run of  PTA $\TA[(x,y),p]$. 
	Let $ \theta=\sup \{ \Gamma(\TA_{\tau})\}.$
	
	If $\theta =\infty$, then  there is a $\nu$ such that $[\nu, \infty) \subseteq \Gamma(\TA_{\tau})$.
	
\end{lemma}

\begin{proof}
\qed
\end{proof}

	
	


\begin{lemma}
\label{lem:oneP4}
Let $\tau=(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_\ell\&a_\ell[u_\ell]}(q_\ell,true)$ 
be a  syntactic run of  PTA $\TA[(x,y),p]$. 
Let $ \gamma \ge S_1$ and  \[\xi= (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_\ell} (q_\ell{,}\omega_\ell)\]
be a run of $\tau[\gamma]$. 
   
    If  $ R(\TA_{\tau[\gamma+1]})=\emptyset$ and $\omega_i'\models g_{i+1}[\gamma+1]$ for $i=0,\cdots, \ell-2$, then  there is a pair $0\le i<j\le \ell$  such that 
   \begin{enumerate}
   
	 \item$a_{i}=a_{j}$;
	\item $u_{i}$ has clock reset about $y$;
	\item $\omega_j(x)-\omega_i(x)> 0$;
	\item there is no $x\succ p$, $x-y\succ p$, $y\succ p$, $y-x\succ p$ in $g_k$, $k\in (i,j]$ .
%	 \item    \[
%	 \begin{split}
%	 \xi_1= &(q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_i} (q_i{,}\omega_i) \\ 
%	   & \xrightarrow{d_i} (q_i{,}\omega_i'^1) \xrightarrow{a_{i+1}} (q_{i+1}{,}\omega_{i+1}^1) \cdots  \xrightarrow{a_j} (q_j{,}\omega_j^1)\\
%	   & \cdots \\
%	   & \xrightarrow{d_i} (q_i{,}\omega_i'^k) \xrightarrow{a_{i+1}} (q_{i+1}{,}\omega_{i+1}^k) \cdots  \xrightarrow{a_j} (q_j{,}\omega_j^k)\\
%	   &   \xrightarrow{d_i} (q_i{,}\omega_i'^*) \xrightarrow{a_{i+1}} (q_{i+1}{,}\omega_{i+1}^*) \cdots  \xrightarrow{a_{\ell}} (q_{\ell}{,}\omega_{\ell}^*)
%	    \end{split}
%	   \]
%	   is a run for syntactic run 
%	    \[
%	    \begin{split}
%	   \tau_1= &(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_i\&a_i[u_i]}(q_i,true) \\ 
%	      & \left(\xrightarrow{g_{i+1}\&a_{i+1}[u_{i+1}]}(q_{i+1},true) {\cdots} \xrightarrow{g_j\&a_j[u_j]}(q_j,true)\right)^k \\
%	     &\xrightarrow{g_{i+1}\&a_{i+1}[u_{i+1}]}(q_{i+1},true) {\cdots} \xrightarrow{g_{\ell}\&a_{\ell}[u_{\ell}]}(q_{\ell},true),
%	    \end{split}
%	    \]
%	    under parameter valuation $\gamma+k\Delta$
%	    where $0<\Delta< S_0,k\in \NN$.
  \end{enumerate}


 \end{lemma}
\begin{proof}
	Let  $\tau_2=(q_0,true)\xrightarrow{g_1\& a_1[u_1]}(q_1,true){\cdots} \xrightarrow{g_{\ell-1}\&a_{\ell-1}[u_{\ell-1}]}(q_{\ell-1},true)$.
	Since $\xi$ is a run of $\tau[\gamma]$ and  $\omega_i'\models g_{i+1}[\gamma+1]$ for $i=0,\cdots, \ell-2$, then $\xi_1$ is a run of
	$\tau_2[\gamma+1]$ where 
	 \[\xi_1= (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_{\ell-1}} (q_{\ell-1}{,}\omega_{\ell-1}).\]
	 Hence there is a conjunct of $g_{\ell}$   with parametric atomic constraint. Since $\omega_{\ell-1}'\models g_{\ell}[\gamma]$ and $\omega_{\ell-1}'\not \models g_{\ell}[\gamma+1] $, there is at least one $x\succ p, y\succ p, -x\succ p, -y\succ p, x-y\succ p$ and
	 $y-x\succ p$ occurring  in $g_\ell$.
	 As $\xi$ is a run of $\tau[\gamma]$ and $\gamma\ge S_1$,  $g_{\ell}$ can not contain $ -x\succ p$ or $ -y\succ p$.
	 It is easy to check that $g_{\ell}$  can not simultaneously contain  $x-y\succ p $ and $y-x\succ p$.
	 
	 \begin{enumerate}
	 	\item  If  $g_\ell$ only contains  $ x\succ p$ and $y\succ p$   in parametric atomic constraints.  In this case,	$\omega_\ell(x)\ge S_1$  and $\omega_\ell(y)\ge S_1$.
	 	According {\em Lemma \ref{lem:oneP6}}, there is a  $0\le h<  \ell$ such that 
	 	\begin{enumerate}
	 		\item $\omega_{h+1}(x)\ge 3S_0\wedge \omega_{h+1}(y)\ge 3S_0$;
	 		\item there is no conjunct of $g_j$ with  parameter-free atomic constraints  $x\prec c$ and $ y\prec c $   where $j\in (h,\ell]$;
	 		\item there is no clocks reset about clocks $x,y$ in $u_j$ where $j\in (h,\ell]$.
	 	\end{enumerate}
	 	Then let 
	 	 \[
	 	 \begin{split}
	 	 \xi_2=& (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots \\
	 	       & \xrightarrow{a_{\ell-1}} (q_{\ell-1}{,}\omega_{\ell-1})\xrightarrow{d_{\ell-1}+1} (q_{\ell-1}{,}\omega_{\ell-1}'+1) \xrightarrow{a_{\ell}} (q_{\ell}{,}\omega_\ell+1).
	 	 \end{split}
	 	 \]
	 	 It is easy to check $\xi_2$ is run for $\tau[\gamma+1]$, which contracts with $R(\TA_{\tau[\gamma+1]})=\emptyset$. Therefore, this case can not occur.

	 	 
	 	 
	 	 
	 	 
	 	 \item If $g_{\ell}$  contains  $x-y\succ p$. 
	 	  As
	 	  $\omega_\ell(x)-\omega_\ell(y)\ge S_1$, employing {\em Lemma \ref{lem:oneP3}},  there is a  $0\le h_1\le h_2<  \ell$ such that 
	 	  \begin{enumerate}
	 	  	  	\item $\omega_{h_1}(x)< S_0\wedge \omega_{h_1+1}(x)\ge S_0$;
	 	  	\item $\omega_{h_2}(x)< 3S_0\wedge \omega_{h_2+1}(x)\ge 3S_0$;
	 	  	\item there is a clocks reset about clock $y$ in $u_j$ where $j\in (h_1,\ell]$;
	 	  	\item there is no clocks reset about clock $x$ in $u_j$ where $j\in (h_1,\ell]$;
	 	  	\item there is no conjunct of $g_j$ with    $x\prec c$    where $j\in (h_1,\ell]$.
	 	  \end{enumerate}
	 	  
	 	  As $\omega_k'(x)< 3S_0, \gamma\ge 4S_0$ and $\xi$ is a run of $\tau[\gamma]$, there is no conjunct of $g_j$ with $x\succ p$ and $x-y\succ p$ for $k\in (h_1,h_2]$. 
	 	  
	 	  {\bf Assume that $h_1=h_2$.} 
	 	  As $d_{h_1}=\omega_{h_1+1}(x)-\omega_{h_1}(x)\ge 2S_0$, $\omega_{h_1}'(y)\ge d_{h_1}\ge 2S_0$.  
	 	  Set $u_k$ be the first clocks reset after $a_{h_1}$ which has reset about $y$. Since $\omega_{k-1}'(y)\ge\omega_{h_1}'(y) \ge 2S_0 $, there is 
	 	  no conjunct of $g_{k}$ in the form of  $y\prec c$ and $-y\succ c$. Thus, $\omega_{k-1}'+1\models g_{k}[\gamma+1]$.
	 	  
	 	  
	 	  \begin{table}
	 	  	\begin{center}	
	 	  		\begin{tabular}{|c|c|c|c|}
	 	  			\hline
	 	  			\cellcolor[gray]{0}
	 	  			$x\prec c$ 	& $x\prec p$ 	&	$x\succ c$ 	& 	\cellcolor[gray]{0} $x\succ p$ \\
	 	  			\hline
	 	  			$y\prec c$ 	& $y\prec p$ 	&  	$y\succ c$ 	& $y\succ p$ \\    
	 	  			\hline
	 	  			$-x\prec c$ 	& $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 		\cellcolor[gray]{0}  $-x\succ p$ \\
	 	  			\hline
	 	  			$-y\prec c$ 	& $-y\prec p$ 	&  	$-y\succ c$ 	& 	\cellcolor[gray]{0} 	$-y\succ p$ \\    
	 	  			\hline
	 	  			$x-y\prec c$ 	& $x-y\prec p$ 	&	$x-y\succ c$ 	&	\cellcolor[gray]{0}  $x-y\succ p$ \\     
	 	  			\hline
	 	  			$y-x\prec c$ 	& $y-x\prec p$ 	&	$y-x\succ c$ 	& $y-x\succ p$\\
	 	  			\hline
	 	  		\end{tabular}
	 	  	\end{center}
	 	  	\caption{All possible atom constraint forms of guard $g_k$ for $k \in (h_1,h_2]$.}
	 	  	\label{tab:9}
	 	  \end{table}
	 	 
%	 	{\bf  Assume that  there is a  $u_k$ has clocks reset about clock $y$ and $\omega_{k-1}'+1\models g_{k}[\gamma+1]$  where $k\in (h_1,\ell]$. }
	 	 Let \[
	 	  \begin{split}
	 	  \xi_3=& (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots  (q_{j-1}{,}\omega_{j-1})\\
	 	  & \xrightarrow{d_{k-1}+1} (q_{k-1}{,}\omega_{k-1}'^*) \xrightarrow{a_{k}} (q_{k}{,}\omega_k^*)\cdots  \xrightarrow{a_{\ell}} (q_{\ell}{,}\omega_\ell^*),
	 	  \end{split}
	 	  \]
	 	  where $\omega_{k-1}'^*=\omega_{k-1}'+1, \omega_\nu^*(x)=\omega_\nu(x)+1, \omega_\nu^*(y)=\omega_\nu(y)$ for $\nu \in [k,\ell]$ and $\omega_\nu'^*(x)=\omega_\nu'(x)+1, \omega_\nu'^*(y)=\omega_\nu'(y)$ for
	 	   $\nu \in [k,\ell)$. Since  $u_k$ has clocks reset about clock $y$ and every constant in $\TA$ is less than $S_0$ and $\omega_k'[x]\ge 3S_0$, $ \omega_\nu'[y]-\omega_\nu'[x]\le -S_0$ for $\nu \in [k,\ell]$. As $\xi$ is a run of $\tau[\gamma]$, there is no 
	 	  conjunct of $g_\nu $ in the form of $y-x\succ c$ or $y-x\succ p$ or $x-y\prec c $ where $\nu \in [k,\ell]$.
	 	   Thus, every conjunct of $g_\nu$ has form 
	 	  among {\em Table \ref{tab:4}}.
	 	  \begin{table}
	 	  	\begin{center}
	 	  		\begin{tabular}{|c|c|c|c|}
	 	  			\hline
	 	  			\cellcolor[gray]{0}
	 	  			$x\prec c$ 	& $x\prec p$ 	&	$x\succ c$ 	& $x\succ p$ \\
	 	  			\hline
	 	  			$y\prec c$ 	& $y\prec p$ 	&  	$y\succ c$ 	& $y\succ p$ \\    
	 	  			\hline
	 	  			$-x\prec c$ 	& $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 	\cellcolor[gray]{0}	 $-x\succ p$ \\
	 	  			\hline
	 	  			$-y\prec c$ 	& $-y\prec p$ 	&  	$-y\succ c$ 	& 	\cellcolor[gray]{0} $-y\succ p$ \\    
	 	  			\hline
	 	  				\cellcolor[gray]{0} $x-y\prec c$ 	& $x-y\prec p$ 	&	$x-y\succ c$ 	& $x-y\succ p$ \\     
	 	  			\hline
	 	  			$y-x\prec c$ 	& $y-x\prec p$ 	& 	\cellcolor[gray]{0}	$y-x\succ c$ 	& 	\cellcolor[gray]{0} $y-x\succ p$\\
	 	  			\hline
	 	  		\end{tabular}
	 	  	\end{center}
	 	  	\caption{All possible atom constraint forms of guard $g_\nu$ for $\nu \in [k,\ell]$ in above.}
	 	  	\label{tab:4}
	 	  \end{table}
	 	  Comparing between $\xi$ and $\xi_3$ after transition $a_k$ only value of $x$ increases $1$ in the same location.
	 	 As  $\omega_i'\models g_{i+1}[\gamma+1]$ for $i=0,\cdots, \ell-2$, all the conjunct of $g_j$ which green color of {\em Table \ref{tab:5}} are satisfied by $\xi_3$ for $j \in [k,\ell)$.
	 	  
	 	  \begin{table}
	 	  	\begin{center}
	 	  		\begin{tabular}{|c|c|c|c|}
	 	  			\hline
	 	  			\cellcolor[gray]{0} 	$x\prec c$ 	& 	 $x\prec p$ 	& 	\cellcolor{green}	$x\succ c$ 	&  \cellcolor{green} $x\succ p$ \\
	 	  			\hline
	 	  			\cellcolor{green} 	$y\prec c$ 	& \cellcolor{green}  $y\prec p$ 	& \cellcolor{green}  	$y\succ c$ 	& \cellcolor{green} $y\succ p$ \\    
	 	  			\hline
	 	  			\cellcolor{green}	$-x\prec c$ 	& \cellcolor{green}  $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 	\cellcolor[gray]{0}	  $-x\succ p$ \\
	 	  			\hline
	 	  			\cellcolor{green}	$-y\prec c$ 	&  \cellcolor{green} $-y\prec p$ 	&  	\cellcolor{green} $-y\succ c$ 	& 	\cellcolor[gray]{0} $-y\succ p$ \\    
	 	  			\hline
	 	  			\cellcolor[gray]{0} $x-y\prec c$ 	&   $x-y\prec p$ 	&  \cellcolor{green}	$x-y\succ c$ 	&  \cellcolor{green}  $x-y\succ p$ \\     
	 	  			\hline
	 	  			\cellcolor{green} $y-x\prec c$ 	&  \cellcolor{green} $y-x\prec p$ 	& 	\cellcolor[gray]{0}	$y-x\succ c$ 	& 	\cellcolor[gray]{0} $y-x\succ p$\\
	 	  			\hline
	 	  		\end{tabular}
	 	  	\end{center}
	 	  	\caption{ The green color label the  partial atom constraint forms in guard $g_j[\gamma+1]$ which satisfied by $\xi_3$ for $j \in [k,\ell)$ in above.}
	 	  	\label{tab:5}
	 	  \end{table}
	 	 
  Since $\omega_k'(x)\models (x\prec p)[\gamma]$, $\omega_k'(x)+1\models (x\prec p)[\gamma+1]$ 
	 	 	for $j \in [k,\ell)$. In other words, conjunct of $g_j$ in the form of $x\prec p$ for $j \in [k,\ell)$ is satisfied by $\omega_{j-1}'^*$ under parameter valuation $\gamma+1$. By the same reason,
	 	 	we can prove that conjunct of $g_j$ in the form of $x-y\prec p$  is satisfied by $\omega_{j-1}'^*$ under parameter valuation $\gamma+1$  for $j \in [k,\ell)$. The result is listed in pink cells of 
	 	 	{\em Table \ref{tab:6}}.
	 	 	
	 	 	
	 	 	
	 	 	  \begin{table}
	 	 	  	\begin{center}
	 	 	  		%\rowcolors{1}{green}{pink}
	 	 	  		
	 	 	  		\begin{tabular}{|c|c|c|c|}
	 	 	  			\hline
	 	 	  			\cellcolor[gray]{0} 	$x\prec c$ 	& 	\cellcolor{pink} $x\prec p$ 	& 	\cellcolor{green}	$x\succ c$ 	& 	\cellcolor{green} $x\succ p$ \\
	 	 	  			\hline
	 	 	  			\cellcolor{green} 	$y\prec c$ 	& \cellcolor{green}  $y\prec p$ 	& \cellcolor{green}  	$y\succ c$ 	& \cellcolor{green} $y\succ p$ \\    
	 	 	  			\hline
	 	 	  			\cellcolor{green}	$-x\prec c$ 	& \cellcolor{green}  $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 	\cellcolor[gray]{0}	  $-x\succ p$ \\
	 	 	  			\hline
	 	 	  			\cellcolor{green}	$-y\prec c$ 	&  \cellcolor{green} $-y\prec p$ 	&  	\cellcolor{green} $-y\succ c$ 	& 	\cellcolor[gray]{0} $-y\succ p$ \\    
	 	 	  			\hline
	 	 	  			\cellcolor[gray]{0} $x-y\prec c$ 	& \cellcolor{pink} $x-y\prec p$ 	&  \cellcolor{green}	$x-y\succ c$ 	&   \cellcolor{green} $x-y\succ p$ \\     
	 	 	  			\hline
	 	 	  			\cellcolor{green} $y-x\prec c$ 	&  \cellcolor{green} $y-x\prec p$ 	& 	\cellcolor[gray]{0}	$y-x\succ c$ 	& 	\cellcolor[gray]{0} $y-x\succ p$\\
	 	 	  			\hline
	 	 	  		\end{tabular}
	 	 	  	\end{center}
	 	 	  	\caption{ The pink color label the  partial atom constraints in guard $g_j[\gamma+1]$ with form  $x\prec p$ or  $x-y\prec p$ which satisfied by $\omega_{j-1}'^*$ for $j \in [k,\ell)$ in above.}
	 	 	  	\label{tab:6}
	 	 	  \end{table}
	 	 	  
	 	 	  If $g_\ell$ contains $x\succ p$,  as $\omega_{\ell-1}'[x]\models (x\succ p)[\gamma]$ and $\omega_{\ell-1}'^*(x)=\omega_{\ell-1}'(x)+1$, $\omega_{\ell-1}'^*(x)\models (x\succ p)[\gamma+1]$. If  $g_\ell$  contains $y\succ p$, then $\omega_{\ell}(x)\ge 3S_0$ and  $\omega_{\ell}(y)\ge 3S_0$.  Through the method of case 1, we can construct $\xi_4$ such that $\xi_4$ is a run of $\tau[\gamma+1]$.
	 	 	
	 	 	
	 	 	Therefore, there is a $\xi_4$
	 	 	  which is a run of $\tau[\gamma+1]$, which contracts with $R(\TA_{\tau[\gamma+1]})=\emptyset$.  So the {\bf assumption} can not hold, i.e.,  
	 	 	  {\bf $h_1<h_2$ and $\omega_{h_2}'(y)< S_0$. } $\omega_{h_2+1}(x)-\omega_{h_1}(x)\ge 2S_0$, there is a clock reset $u_k$ about $y$ where 
	 	 	  $k\in (h_1,h_2]$. 
	 	 	  
	 	 	  
	 	 	  {\bf Assume that there is $u_j$ has clocks reset about clock $y$  where $j\in (h_1,h_2]$ such that $\omega_{j-1}'+1\not \models g_{j}[\gamma+1]$ when  $u_j$ has clocks reset about clock $y$  where $j\in (h_1,h_2]$. } Then by the above procedure, we also  can construct a $\xi_5$
	 	 	  which is a run of $\tau[\gamma+1]$.
	 	 	  
	 	 	  
	 	 	  
	 	 	   Hence, $\omega_{j-1}'+1\not \models g_{j}[\gamma+1]$ when  $u_j$ has clocks reset about clock $y$  where $j\in (h_1,h_2]$.  Hence, $g_j$ has conjunct $y\prec c$  or $-y\succ c$ and has not conjunct $y\succ p$ when  $u_j$ has clocks reset about clock $y$  where $j\in (h_1,h_2]$. As the only possibility method to reduce  value of expression  $y$ in $\xi$ is encountering  {\em instantaneous transition} $a_j$ with $u_j$ which 
	 	 	  has clocks reset about clock $y$. For every  {\em instantaneous transition}  $a_j$ with $u_j$ which 
	 	 	  has clocks reset about clock $y$, the value of expression $y$ reduce at most $2\maxC(\TA)$. Since $\left(\omega_{h_2+1}(x)-\omega_{h_1}(x)\right)\ge 2S_0$. By {\em Pigeonhole principle}, there is a pair $0\le h_1< i<j\le h_2$  such that $a_{i}=a_{j}, \omega_j(x)-\omega_i(x)> 0$ and  $u_{i}$  
	 	 	  has clocks reset about clock $y$.
	 	 	  % Let $\Delta=\omega_j(x)-\omega_i(x) $.
	 	 	  
%	 	 	   \begin{table}
%	 	 	   	\begin{center}
%	 	 	   		\begin{tabular}{|c|c|c|c|}
%	 	 	   			\hline
%	 	 	   			\cellcolor[gray]{0}
%	 	 	   			$x\prec c$ 	& $x\prec p$ 	&	$x\succ c$ 	& $x\succ p$ \\
%	 	 	   			\hline
%	 	 	   		\cellcolor{red}	$y\prec c$ 	& $y\prec p$ 	&  	$y\succ c$ 	& 	\cellcolor[gray]{0} $y\succ p$ \\    
%	 	 	   			\hline
%	 	 	   			$-x\prec c$ 	& $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 	\cellcolor[gray]{0}	 $-x\succ p$ \\
%	 	 	   			\hline
%	 	 	   			$-y\prec c$ 	& $-y\prec p$ 	&  \cellcolor{red}	$-y\succ c$ 	& 	\cellcolor[gray]{0}  $-y\succ p$ \\    
%	 	 	   			\hline
%	 	 	   			\cellcolor[gray]{0} $x-y\prec c$ 	& $x-y\prec p$ 	&	$x-y\succ c$ 	& $x-y\succ p$ \\     
%	 	 	   			\hline
%	 	 	   			$y-x\prec c$ 	& $y-x\prec p$ 	& 	\cellcolor[gray]{0}	$y-x\succ c$ 	& 	\cellcolor[gray]{0} $y-x\succ p$\\
%	 	 	   			\hline
%	 	 	   		\end{tabular}
%	 	 	   	\end{center}
%	 	 	   	\caption{$g_j$ has conjunct $y\prec c$  or $-y\succ c$  when  $u_j$ has clocks reset about clock $y$  where $j\in (h,\ell]$.}
%	 	 	   	\label{tab:7}
%	 	 	   \end{table}
%	 	 	   
%	 	 	   
%	 	 	   
%	 	 	    \begin{table}
%	 	 	    	\begin{center}
%	 	 	    		\begin{tabular}{|c|c|c|c|}
%	 	 	    			\hline
%	 	 	    			\cellcolor[gray]{0}
%	 	 	    			$x\prec c$ 	& 	\cellcolor{green} $x\prec p$ 	&	\cellcolor{green} $x\succ c$ 	& $x\succ p$ \\
%	 	 	    			\hline
%	 	 	    			\cellcolor{green}	$y\prec c$ 	& \cellcolor{green} $y\prec p$ 	&  	\cellcolor{green} $y\succ c$ 	& 	\cellcolor[gray]{0} $y\succ p$ \\    
%	 	 	    			\hline
%	 	 	    			\cellcolor{green} $-x\prec c$ 	& \cellcolor{green} $-x\prec p$ 	& 	\cellcolor[gray]{0}	$-x\succ c$ 	& 	\cellcolor[gray]{0}	 $-x\succ p$ \\
%	 	 	    			\hline
%	 	 	    		\cellcolor{green} 	$-y\prec c$ 	& \cellcolor{green} $-y\prec p$ 	&  \cellcolor{green}	$-y\succ c$ 	& 	\cellcolor[gray]{0} $-y\succ p$ \\    
%	 	 	    			\hline
%	 	 	    			\cellcolor[gray]{0} $x-y\prec c$ 	& \cellcolor{green} $x-y\prec p$ 	& \cellcolor{green}	$x-y\succ c$ 	& $x-y\succ p$ \\     
%	 	 	    			\hline
%	 	 	    		\cellcolor{green}	$y-x\prec c$ 	& \cellcolor{green} $y-x\prec p$ 	& 	\cellcolor[gray]{0}	$y-x\succ c$ 	& 	\cellcolor[gray]{0} $y-x\succ p$\\
%	 	 	    			\hline
%	 	 	    		\end{tabular}
%	 	 	    	\end{center}
%	 	 	    	\caption{parameter valuation $\gamma+k\Delta$.}
%	 	 	    	\label{tab:8}
%	 	 	    \end{table}
%%
%	 	
%	 	 \ly{
%hhhhhhhhhhhhhhhhhh	 	 }
%	 
%	 	 In this case	$\omega_\ell(x)\ge 3S_0$  and $\omega_\ell(y)\ge 3S_0$.
%	 	 According {\em Lemma \ref{lem:oneP6}}, 
%	 	 $\omega_\ell(x)\ge 3S_0$  and $\omega_\ell(y)\ge 3S_0$ there is a  $0\le i<  \ell$ such that 
%	 	 \begin{enumerate}
%	 	 	\item $\omega_{i+1}(x)\ge 2S_0\wedge \omega_{i+1}(y)\ge 2S_0$;
%	 	 	\item there is no conjunct of $g_j$ with  parameter-free atomic constraints  $x\prec c$ and $ y\prec c $   where $j\in (i,\ell]$;
%	 	 	\item there is no clocks reset about clocks $x,y$ in $u_j$ where $j\in (i,\ell]$.
%	 	 \end{enumerate}
%	 	 Then   let 
%	 	 \[
%	 	 \begin{split}
%	 	 \xi_2=& (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots \\
%	 	 & \xrightarrow{a_{\ell-1}} (q_{\ell-1}{,}\omega_{\ell-1})\xrightarrow{d_{\ell-1}+1} (q_{\ell-1}{,}\omega_{\ell}'+1) \xrightarrow{a_{\ell}} (q_{\ell}{,}\omega_\ell+1).
%	 	 \end{split}
%	 	 \]
%	 	 
%	 	 Since $\omega_{\ell-1}'\models  g_{\ell}[\gamma]$, $\omega_{\ell-1}'+1\models   \left(x\succ p\wedge y\succ p\right)[\gamma+1]$. 
	 \end{enumerate}
	\qed 
	 
	
%	
%	Since $\gamma\ge 3S_0$, 
%	
%If $\theta< \infty$. In other words, there is a run
%  \[\xi= (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots   \xrightarrow{a_\ell} (q_\ell{,}\omega_\ell)\]
% of $\tau[\theta]$ such that $\omega_\ell(x)-\omega_\ell(y)\succ \theta\ge 3S_0$.
%According {\em Lemma \ref{lem:oneP3}}, there is a   $k$  such that
%\begin{enumerate}
%\item $\omega_k(x)< 2S_0\wedge \omega_{k+1}(x)\ge 2S_0$;
%\item there is a clocks reset about clock $y$ in $a_h$ where $h\in (k,\ell]$;
%\item there is no clocks reset about clock $x$ in $a_h$ where $h\in (k,\ell]$.
%\end{enumerate}
%As  $\omega_\mu\ge 2S_0$ for $\mu\in (k,\ell]$ and $S_0$ is greater than each constant occurring in $\TA$, there is no  parameter-free atomic constraints with form $x\prec c$ in transition $a_h$ for $h\in (k,\ell]$.  Set the $a_\mu$ has  clocks reset about clock $y$ where $\mu\in (k,\ell]$.
%
% Assume there is no conjunct of $a_\mu$ has form parameter-free atomic constraints $y\prec c$.
%  Let
%\[
%\begin{split}
%\xi'=& (q_0{,}\omega_0)\xrightarrow{d_0} (q_0{,}\omega_0') \xrightarrow{a_1} (q_1{,}\omega_1) \cdots  (q_{\mu-1}{,}\omega_{\mu-1})
%\xrightarrow{d_{\mu-1}+1} (q_{\mu-1}{,}\omega_{\mu-1}'^*) \\ &\xrightarrow{a_\mu} (q_\mu{,}\omega_\mu^*)  \cdots   \xrightarrow{a_\ell} 
%(q_\ell{,}\omega_\ell^*)
%\end{split}
% \]
% where $\omega_{h}'^*(x)=\omega_{h}'(x)+1$ for $h\in [\mu-1,\ell)$,  $\omega_{h}^*(x)=\omega_{h}(x)+1$ for $h \in [\mu, \ell]$, $\omega_{\mu-1}'^*(y)=\omega_{\mu-1}'(y)+1$,  $\omega_{\mu-1}'^*(y)=\omega_{\mu-1}'(y)$ for $h \in [\mu, \ell)$ and 
% $  \omega_{h}^*(y)=\omega_{h}(y)$ for $h \in [\mu, \ell]$.
% It is easy to check that $\xi'$
% is a run of $\tau[\gamma^*+1]$. Which contracts with the definition of $\theta$.


\end{proof}



\begin{lemma}
Let   $\TA[(x,y),p]$ be a two-one PTA and  $\psi$ be   $\forall \Box \phi$. If there is a $T\ge S_1$ such that
$\TA[p=T]\models \psi$, then there are $T_1\in [S_1, S_1+S_0]$ and $c\le S_0$ such that $\TA[p=T_1+kc]\models \psi$ for $k\in \NN$.
\end{lemma}

\begin{proof}
Let $\tau=q_0\xrightarrow{g_1\&a_1}q_1\cdots \xrightarrow{g_\ell\& a_\ell}q_\ell$ be a  syntactic run of  PTA $\TA[(x,y),p]$ such that 
$\tau[p=T]\models \psi$. According {\em Lemma \ref{lem:moveI}}, we can obtain a syntactic run $\beta(\tau)$ such that 
$\tau[\gamma]\models \psi$ equivalents to $R(\TA_{\beta(\tau)}[\gamma])\neq \emptyset$ for each parameter valuation $\gamma$.

If $\tau$ does not contains  parametric constraint, then value of $p$ can not influence $\tau$. Thus, $\tau[\gamma]\models$ for $p\in \NN$.
Therefore, the conclusion holds in this case. 

If  there is no clocks reset in $\beta(\tau)$, employing {\em Lemma \ref{lem:oneP1}}, $R(\TA_{\beta(\tau)}[p=T])\neq \emptyset$
for $T\ge S_1$. Thus, the conclusion holds in this case.

\qed
\end{proof}


%
%\begin{lemma}
%	\label{lem:oneP2}
%	Let $\tau$ be a  syntactic  run of a two-one PTA $\mathcal{A}[(x,y),p]$ without location invariants.  
%	 The set $\Gamma(\TA_{\tau})$ is solvable if there is one guard of $\tau$ with parameter. 
%\end{lemma}
%\begin{proof}
%
%\qed
%\end{proof}


